An Integrated Visual Analytics System for Studying Clinical Carotid Artery Plaques

Carotid artery plaques can cause arterial vascular diseases such as stroke and myocardial infarction, posing a severe threat to human life. However, the current clinical examination mainly relies on a direct assessment by physicians of patients' clinical indicators and medical images, lacking an integrated visualization tool for analyzing the influencing factors and composition of carotid artery plaques. We have designed an intelligent carotid artery plaque visual analysis system for vascular surgery experts to comprehensively analyze the clinical physiological and imaging indicators of carotid artery diseases. The system mainly includes two functions: First, it displays the correlation between carotid artery plaque and various factors through a series of information visualization methods and integrates the analysis of patient physiological indicator data. Second, it enhances the interface guidance analysis of the inherent correlation between the components of carotid artery plaque through machine learning and displays the spatial distribution of the plaque on medical images. Additionally, we conducted two case studies on carotid artery plaques using real data obtained from a hospital, and the results indicate that our designed carotid analysis system can effectively provide clinical diagnosis and treatment guidance for vascular surgeons.

==> 00_acknowledgement.tex <==
This research is sponsored in part by the U.S. National Science Foundation through grants IIS-1528203 and IIS-1741536, and the Nature Science Foundation of China through grant 61976075.
 
We thank Dr. Pauline Maillard from the Department of Neurology, the University of California at Davis, Dr. Xiufang Xu from Hangzhou Medical College, and Dr. Chao Lin from the Children's Hospital of Zhejiang University School of Medicine who provided insight and expertise that greatly assisted the research. We would also like to show our gratitude to Dr. Shunyuan Guo and Dr. Gaoping Lin from Zhejiang Provincial People’s Hospital for sharing their pearls of wisdom with us during this research.

Data used in the preparation of this article were obtained from the
Parkinson's Progression Markers Initiative (PPMI) database (\url{www.ppmiinfo.org/data}). For up-to-date information on the study, visit \url{www.ppmiinfo.org}.
PPMI---a public-private partnership---is funded by the Michael J. Fox Foundation
for Parkinson’s Research and funding partners, including AbbVie, Allergan, Avid Radiopharmaceuticals, Biogen, BioLegend, Bristol-Myers Squibb, Celgene, Covance, GE Healthcare, Genentech, GlaxoSmithKline, Golub Capital, Handl Therapeutics, Insitro, Lilly, Lundbeck, Merck, Meso Scale Discovery, Pfizer, Piramal, Prevail, Roche, Roche, Sanofi Genzyme, Servier, Takeda, TEVA, UCB, Verily, and Voyager.

==> 00_biography.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{BioPhotos/ChaoqingXu.jpg}}]%
    {Chaoqing Xu} received the BS degree in automation from Zhejiang University of Science and Technology. He is a Ph.D. student in control science and engineering from the Zhejiang University of Technology, Hangzhou, China. He was a  visiting scholar at the University of California, Davis, from January 2017 to October 2018. He is currently working with Ronghua Liang. His main research interests include medical visualization and brain fiber analysis.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{BioPhotos/Tyson.jpg}}]%
    {Tyson Neuroth} received the BS degree in computer science from the University of California, Davis. He is now a Ph.D. student at the University of California, Davis, studying computer science and visualization under Kwan-Liu Ma. His research interests include scientific visualization, high performance computing, and human-computer interaction. 
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{BioPhotos/Takanori.jpg}}]%
    {Takanori Fujiwara} received his Ph.D. degree in computer science at the University of California, Davis in 2021. Before UC Davis, he received his Master's degree in environmental studies in 2011 from the University of Tokyo and worked for Kajima Corporation in Japan. He works at the intersection of data science and data visualization with special interests in visual analytics using machine learning for high-dimensional and network data. 
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{BioPhotos/RonghuaLiang.jpg}}]%
    {Ronghua Liang} received the PhD degree in computer science from Zhejiang University in 2003. He was a research fellow at the University of Bedfordshire, United Kingdom, from April 2004 to July 2005 and as a visiting scholar at the University of California, Davis, from March 2010 to March 2011. He is currently a professor of computer science and dean of the College of Computer Science and Technology, Zhejiang University of Technology, China. He has published more than 80 papers in leading international journals and conferences including IEEE Transactions on Knowledge and Data Engineering, IEEE Transactions on Visualization and Computer Graphics, IEEE Information Visualization, IJCAI, AAAI. His research interests include medical visualization, image processing, and big data visualization. He is a member of the IEEE.
\end{IEEEbiography}
 
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{BioPhotos/KwanLiuMa_portrait010.jpg}}]%
    {Kwan-Liu Ma} is a distinguished professor of computer science at the University of California, Davis. He received his PhD degree in computer science from the University of Utah in 1993, and then worked as a staff scientist at ICASE/NASA Langley Research Center before joining UC Davis in 1999.  His research is in the intersection of data visualization, computer graphics, human-computer interaction, and high performance computing.  For his significant research accomplishments, Ma received several recognitions including elected as IEEE Fellow in 2012, recipient of the IEEE VGTC Visualization Technical Achievement Award in 2013, and inducted to IEEE Visualization Academy in 2019.
\end{IEEEbiography}


